SV3D: Novel Multi-view Synthesis and 3D Generation from a Single Image using Latent Video Diffusion

We present Stable Video 3D (SV3D) -- a latent video diffusion model for high-resolution, image-to-multi-view generation of orbital videos around a 3D object. Recent work on 3D generation propose techniques to adapt 2D generative models for novel view synthesis (NVS) and 3D optimization. However, these methods have several disadvantages due to either limited views or inconsistent NVS, thereby affecting the performance of 3D object generation. In this work, we propose SV3D that adapts image-to-video diffusion model for novel multi-view synthesis and 3D generation, thereby leveraging the generalization and multi-view consistency of the video models, while further adding explicit camera control for NVS. We also propose improved 3D optimization techniques to use SV3D and its NVS outputs for image-to-3D generation. Extensive experimental results on multiple datasets with 2D and 3D metrics as well as user study demonstrate SV3D's state-of-the-art performance on NVS as well as 3D reconstruction compared to prior works.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/appendices/B.tex <==
\section{Related Work}
\label{supsec:related_work}

\textbf{Video Synthesis.} 
%Due to its computational demands, 
%and a lack of publicly available data, 
%video synthesis has not been among the most investigated research areas for several years. However, 
Many approaches based on various models such as variational RNNs~\cite{babaeizadeh2018stochastic,svg,lee2018savp,hvrnn,lsvg}, normalizing flows~\citep{si2v,ipoke}, autoregressive transformers~\cite{Weissenborn2020Scaling,yan2021videogpt,hong2022cogvideo,wu2021godiva,wu2022nuwa,ge2022longvideo,Gupta_2022_CVPR}, and GANs~\citep{scene_dyn,yu2022generating,tian2021a, villegas17mcnet,Luc2020TransformationbasedAV,TGAN2020,brooks2022generating,Skorokhodov_2022_CVPR,kahembwe2020lower,TGAN2017,Wang_2020_CVPR,fox2021stylevideogan} have tackled video synthesis. Most of these works, however, have generated videos either on low-resolution~\citep{babaeizadeh2018stochastic,svg,lee2018savp,hvrnn,lsvg,si2v,ipoke,scene_dyn,yu2022generating,tian2021a, villegas17mcnet,Luc2020TransformationbasedAV} or on comparably small and noisy datasets~\cite{carreira2017quo,soomro2012ucf101,xu2016msr-vtt} which were originally proposed to train discriminative models. 

Driven by increasing amounts of available compute resources and datasets better suited for generative modeling such as WebVid-10M~\citep{bain2022frozen}, more competitive approaches have been proposed recently, mainly based on well-scalable, explicit likelihood-based approaches such as diffusion~\cite{ho2022video,singer2022make,ho2022imagenvideo} and autoregressive models~\citep{villegas2022phenaki}. Motivated by a lack of available clean video data, all these approaches are leveraging joint image-video training~\citep{singer2022make,ho2022imagenvideo,zhou2022magicvideo,blattmann2023align} and most methods are grounding their models on pretrained image models~\citep{singer2022make,zhou2022magicvideo,blattmann2023align}. Another commonality between these and most subsequent approaches to (text-to-)video synthesis~\cite{ge2023preserve,wang2023modelscope,wang2023lavie} is the usage of dedicated expert models to generate the actual visual content at a coarse frame rate and to temporally upscale this low-fps video to temporally smooth final outputs at 24-32 fps~\citep{singer2022make,ho2022imagenvideo,blattmann2023align}. Similar to the image domain, diffusion-based approaches can be mainly separated into cascaded approaches~\citep{ho2022imagenvideo} following~\citep{ho2021cascaded,ge2023preserve} and latent diffusion models~\citep{blattmann2023align,zhou2022magicvideo,zhang2023i2vgen} translating the approach of \citet{rombach2021high} to the video domain. While most of these works aim at learning general motion representation and are consequently trained on large and diverse datasets, another well-recognized branch of diffusion-based video synthesis tackles personalized video generation based on finetuning of pretrained text-to-image models on more narrow datasets tailored to a specific domain~\citep{guo2023animatediff} or application, partly including non-deep motion priors~\citep{zhang2023i2vgen}. Finally, many recent works tackle the task of image-to-video synthesis, where the start frame is already given, and the model has to generate the consecutive frames~\cite{zhang2023i2vgen,wang2023modelscope,guo2023animatediff}. Importantly, as shown in our work (see~\Cref{fig:teaser}) when combined with off-the-shelf text-to-image models, image-to-video models can be used to obtain a full text-(to-image)-to-video pipeline.   

% \textbf{New papers after Video LDM}
% Nvidia video paper\citet{ge2023preserve}, Animate Diff \citet{guo2023animatediff}, ModelScope\cite{wang2023modelscope}, \citet{geyer2023tokenflow}, LAVIE model\citet{wang2023lavie}, GAIA driving model \cite{hu2023gaia}, MAGVIT-v2 \citet{yu2023language}, \cite{wang2023videofactory}, Show1 model \cite{zhang2023show}, ``we investigate how to adapt a large pretrained text-to-video model to a variety of downstream domains and tasks without finetuning'' \citet{yang2023probabilistic}, I2VGen-XL \citet{zhang2023i2vgen}, EvalCrafter \citet{liu2023evalcrafter}, Similar to Andi's poking paper but for diffusion \citet{chen2023motion}


% \TODO{NEEDS HEAVY REPHRASING}
% Most related to our work are previous DMs for video synthesis:
% \citet{ho2022video} model low-resolution videos with DMs in pixel space and train jointly on image and video data. \citet{yang2022video} parameterize autoregressive video generation using a deterministic frame predictor together with a probabilistic diffusion model. \citet{voleti2022mcvd} present a general diffusion model framework that simultaneously enables video generation, prediction and interpolation, similar to ~\citet{hoeppe2022diffusion}. \citet{harvey2022flexible} synthesize long videos by first generating sparse images and then adding the missing images.

% Various non-diffusion based approaches have been employed for video generation, utilizing, for example, recurrent neural networks~\cite{babaeizadeh2018stochastic,svg,lee2018savp,hvrnn,lsvg}, autoregressive transformers~\cite{Weissenborn2020Scaling,yan2021videogpt,hong2022cogvideo,wu2021godiva,wu2022nuwa,ge2022longvideo,Gupta_2022_CVPR}, Normalizing Flows~\cite{si2v,ipoke}, and generative adversarial networks (GANs)\cite{scene_dyn,yu2022generating,tian2021a, villegas17mcnet,Luc2020TransformationbasedAV,TGAN2020,brooks2022generating,Skorokhodov_2022_CVPR,kahembwe2020lower,TGAN2017,Wang_2020_CVPR,fox2021stylevideogan}. 
% Temporal layers in pretrained generators have been explored by GAN-based methods like MoCoGAN-HD~\cite{tian2021a} and StyleVideoGAN~\cite{fox2021stylevideogan}, albeit on a smaller scale for object-centric videos. LongVideoGAN\cite{brooks2022generating} demonstrated success in high-resolution video synthesis across extended time intervals by combining low- and high-resolution models. 
% CogVideo~\cite{hong2022cogvideo} finetunes a discrete, autoregressive text-to-image model for video generation. 
% %In contrast, our method relies on continuous distributional models (DMs), demonstrating lower parameter intensity and superior performance in text-to-video synthesis compared to CogVideo. %Additionally, our alignment layers are implemented differently, eliminating the need for autoregressive masking and conditioning on text prompts for text-to-video experiments.
% Numerous other text-to-video models exist~\cite{mittal2017sync,Pan2017ToCW,marwah2017attentive,li2017video,gupta2018imagine,wu2021godiva,wu2022nuwa}.

% Video generation has been tackled with recurrent neural networks~\cite{babaeizadeh2018stochastic,svg,lee2018savp,hvrnn,lsvg}, autoregressive transformers~\cite{Weissenborn2020Scaling,yan2021videogpt,hong2022cogvideo,wu2021godiva,wu2022nuwa,ge2022longvideo,Gupta_2022_CVPR}, Normalizing Flows~\cite{si2v,ipoke}, and generative adversarial networks (GANs)~\cite{scene_dyn,yu2022generating,tian2021a, villegas17mcnet,Luc2020TransformationbasedAV,TGAN2020,brooks2022generating,Skorokhodov_2022_CVPR,kahembwe2020lower,TGAN2017,Wang_2020_CVPR,fox2021stylevideogan}. In particular LongVideoGAN~\cite{brooks2022generating} achieves high-resolution video synthesis over relatively long time intervals, combining a low- and a high-resolution model. Moreover, the idea to insert temporal layers into pretrained generators has been explored by the GAN-based methods MoCoGAN-HD~\cite{tian2021a} and StyleVideoGAN~\cite{fox2021stylevideogan} before, but at a much smaller scale for simple object-centric videos.
% Another important work is CogVideo~\cite{hong2022cogvideo}, which video fine-tunes a text-to-image model. 
% %
% %
% However, it is a strictly autoregressive architecture building on transformers, trained in a discrete latent space. Our method, in contrast, relies on continuous DMs, is much less parameter intensive and outperforms CogVideo in text-to-video synthesis. Furthermore, our alignment layers are also implemented differently. They do not require an autoregressive masking and, for our text-to-video experiments, condition on the text prompts.
% Finally, we also show driving scene generation, where we employ an additional video fine-tuned upsampler module. Many more text-to-video models exist~\cite{mittal2017sync,Pan2017ToCW,marwah2017attentive,li2017video,gupta2018imagine,wu2021godiva,wu2022nuwa,ho2022video}.



% \textbf{Concurrent Work.}\TODO{Shorten significantly and merge with the above} \textbf{Copy \& Pasted from VideoLDM}. Concurrently with us, Make-A-Video~\cite{singer2022make} leveraged a DALL$\cdot$E 2-like text-to-image DM~\cite{ramesh2022dalle2} and temporally aligned its decoder as well as one super resolution DM for consistent video generation. Furthermore, Imagen Video~\cite{ho2022imagenvideo} trained a large-scale cascaded text-to-video model building on the Imagen~\cite{saharia2022imagen} architecture. It constructs a highly demanding spatial and temporal super resolution pipeline consisting of in total 7 DMs with a total of ${>}11$B parameters (also see model parameters comparisons in \Cref{app:model_params}).
% In contrast to our Video LDM, both Imagen Video and Make-A-Video operate entirely in pixel space, which is less efficient, and exclusively target text-to-video, whereas we also demonstrate high-resolution driving scene generation. 
% Furthermore, neither the large-scale DALL$\cdot$E 2 and Imagen text-to-image models, nor the corresponding text-to-video models are easily reproducible without substantial GPU resources. In contrast, we are building on \emph{Stable Diffusion} to train our text-to-video model, and construct an overall significantly more efficient pipeline. This makes our approach more user-friendly. 
% Phenaki~\cite{villegas2022phenaki} is another strong concurrent text-to-video model that compresses videos into discrete tokens and models the token distribution via bidirectional transformers. MagicVideo~\cite{zhou2022magicvideo} is a concurrent method that also leverages latent diffusion models for video generation and follows a partially related strategy compared to our Video LDM. We are outperforming MagicVideo quantitatively (see \Cref{sec:text-to-video}), enable higher resolution generation, show personalized video generation, and also demonstrate long driving scene and mountain bike video generation; in contrast, MagicVideo tackles text-to-video only. Other relevant concurrent works include GEN-1~\cite{esser2023structure}, which also leverages a latent diffusion framework and combines it with depth conditioning for structure- and content-aware video editing and stylization, as well as Dreamix~\cite{molad2023dreamix}, a method for video editing that demonstrates personalized video generation.

\textbf{Multi-View Generation}
Motivated by their success in 2D image generation, diffusion models have also been used for multi-view generation. Early promising diffusion-based results~\citep{watson2022novel,zhou2023sparsefusion,anciukevivcius2023renderdiffusion,nichol2022pointe,jun2023shape,deng2023nerdi} have mainly been restricted by lacking availability of useful real-world multi-view training data.     
To address this, more recent works such as Zero-123~\cite{liu2023zero1to3}, MVDream~\cite{shi2023mvdream}, and SyncDreamer~\cite{liu2023syncdreamer} propose techniques to adapt and finetune pretrained image generation models such as Stable Diffusion (SD) for multi-view generation, thereby leveraging image priors from SD.
% %% Multi-view generation problem and current techniques
% A typical 3D object reconstruction pipeline first involves capturing the multi-view images of an object followed by 3D optimization (e.g., NeRF~\cite{}).
% Following this protocol for generation, several recent works~\cite{zero123, zero123xl} propose techniques to 
% \textit{generate} multiple views of an object from a single image thereby facilitating the 3D asset generation from a given text or single object image. These works adapt the image generation models such as Stable Diffusion (SD)~\cite{} by adding a camera pose-conditioning thereby leveraging the generic image generation priors from SD. A typical strategy is to 
% fine-tune the image generation model on multi-view image datasets such as Objaverse~\cite{}. 
One issue with Zero-123~\cite{liu2023zero1to3} is that the generated multi-views can be inconsistent with respect to each other as they are generated independently with pose-conditioning. 
Some follow-up works try to address this view-consistency problem by jointly synthesizing the multi-view images. MVDream~\cite{shi2023mvdream} proposes to jointly generate four views of an object using a shared attention module across images. SyncDreamer~\cite{liu2023syncdreamer} proposes to estimate a 3D voxel structure in parallel to the multi-view image diffusion process to maintain consistency across the generated views.


%% Video models are more suitable for multi-view generation
Despite rapid progress in multi-view generation research, these approaches rely on single image generation models such as SD. We believe that our video generative model is a better candidate for the multi-view generation as multi-view images form a specific form of video where the camera is moving around an object. As a result, it is much easier to adapt a video-generative model for multi-view generation compared to adapting an image-generative model. In addition, the temporal attention layers in our video model naturally assist in the generation of consistent multi-views of an object without needing any explicit 3D structures like in~\cite{liu2023syncdreamer}.


==> sec/appendices/C.tex <==
\section{\textbf{Data Processing}}
\label{supsec:data_proc}
In this section, we provide more details about our processing pipeline including their outputs on a few public video examples for demonstration purposes. 
%All these visual examples are available on YouTube under a CC-license. We include the URL of each video example in the respective visualization.  

\paragraph{Motivation}
We start from a large collection of raw video data which is not useful for generative text-video (pre)training~\citep{ramesh2022hierarchical,wang2023internvid} because of the following adverse properties: First, in contrast to discriminative approaches to video modeling, generative video models are sensitive to motion inconsistencies such as cuts of which usually many are contained in raw and unprocessed video data, \cf \Cref{fig:cuts_and_motion}, left. Moreover, our initial data collection is biased towards still videos as indicated by the peak at zero motion in \Cref{fig:cuts_and_motion}, right. Since generative models trained on this data would obviously learn to generate videos containing cuts and still scenes, this emphasizes the need for cut detection and motion annotations to ensure temporal quality. Another critical ingredient for training generative text-video models are captions - ideally more than one per video~\citep{somepalli2023understanding} - which are well-aligned with the video content. The last essential component for generative video training which we are considering here is the high visual quality of the training examples.  

The design of our processing pipeline addresses the above points. Thus, to ensure temporal quality, we detect cuts with a cascaded approach directly after download, clip the videos accordingly, and estimate optical flow for each resulting video clip. After that, we apply three synthetic captioners to every clip and further extract frame-level CLIP similarities to all of these text prompts to be able to filter out outliers. Finally, visual quality at the frame level is assessed by using a CLIP-embeddings-based aesthetics score~\citep{schuhmann2022laion}. We describe each step in more detail in what follows.


% To instantiate our dataset we download the videos at native resolution, perform scene detection, and key-frame aware clipping \ref{keyframeaware}
% according to the detected scenes. The scene detection and clipping combination is useful for creating good quality video clips, however this creates the issue of losing unique metadata for each video since now we have multiple samples which come from the same base video and therefore share the same internet sourced metadata. One could use the subtitles that occur during a given clip as the text caption however this has its limitations. YouTube auto-generated subtitles are known to not have great quality and alignment and additionally audio transcripts rarely describe the \textit{visual} features that are occurring during a given time. To solve this issue we create synthetic captions which target visual and temporal descriptions for each clip. Additionally we collect the available YouTube metadata and compute and optical flow estimates for each clip. Below, we go into details on each of these transformations.
\cutsfadesvis

\paragraph{Cascaded Cut Detection.}
Similar to previous work~\citep{wang2023internvid}, we use PySceneDetect~\footnote{\url{https://github.com/Breakthrough/PySceneDetect}} to detect cuts in our base video clips. However, as qualitatively shown in \Cref{fig:cuts_fades} we observe many fade-ins and fade-outs between consecutive scenes, which are not detected when running the cut detector at a unique threshold and only native fps. Thus, in contrast to previous work, we apply a cascade of 3 cut detectors which are operating at different frame rates and different thresholds to detect both sudden changes and slow ones such as fades. 

% We clip the video frames with FFMPEG~\citep{tomar2006converting} directly after cut detection.

\paragraph{Keyframe-Aware Clipping.} We clip the videos using FFMPEG~\citep{tomar2006converting} directly after cut detection by extracting the timestamps of the keyframes in the source videos and snapping detected cuts onto the closest keyframe timestamp, which does not cross the detected cut. This allows us to quickly extract clips without cuts via seeking and isn't prohibitively slow at scale like inserting new keyframes in each video.

% We make use of the content-aware scene detection functionality of the PySceneDetect python package to detect scenes in videos and return their time ranges. This is parameterized by 2 arguments - a  threshold which controls the average change in pixel intensity required to trigger a cut and a minimum scene length (measured in frames). For our dataset, we chose to err on the side of caution, and set very aggressive thresholds for scene detection, choosing a threshold of 11.5. This has the effect of introducing unnecessary cuts in response to some motion, creating many extraneous small clips. So to combat this we filter all videos under 4 seconds long. % \todo{find info about those experiments we did early on and report here (I'm worried they might've had something to do with optical flow which was bad in those times)}


\staticvis
\paragraph{Optical Flow.} 
As motivated in \Cref{subsec:data_proc} and \Cref{fig:cuts_and_motion} it is crucial to provide means for filtering out static scenes. To enable this, we extract dense optical flow maps at 2 FPS using the OpenCV~\citep{itseez2015opencv} implementation of the Farneb\"ack algorithm~\citep{farneback2003flow}. To further keep storage size tractable, we spatially downscale the flow maps such that the shortest side is at 16px resolution. By averaging the flow vector magnitude over time and spatial coordinates, we further obtain a global motion score for each clip, which we use to filter out static scenes by using a threshold for the minimum required motion, which is chosen as detailed on \Cref{supsubsec:filtering_ablations}. Since this only yields rough approximate, for the final Stage III finetuning, we compute more accurate dense optical flow maps using RAFT~\cite{teed2020raft} at $800 \times 450$ resolution at 4 FPS. The motion scores are then computed similarly and scaled (divided) by a factor of 28.125 to match the distribution of pretraining data. Since the high-quality finetuning data is relatively much smaller than the pretraining dataset, this makes the RAFT-based flow computation tractable. Empirically, most motion score estimates computed by this method lie in the 0.0-3.5 range, with some scores over that. We divide this range of 0.0-3.5 into 1024 buckets and condition our model on the bucket ID where the motion scores lie, with values over 3.5 getting mapped to the last bucket.  



% We use the OpenCV python package to compute the Gunnar-Farneback optical flow for each clip. In order to make this operation cheaper and metadata size smaller we downsample the input videos such that the shortest side is 16px, and we also temporally downsample to 2fps. We save the mean of the optical flow magnitudes across the spatial dimension and the entire video to produce a per-frame motion estimate and a per-clip motion estimate which can be easily used to filter the dataset based on desired amount of movement in videos. For example, one could set a minimal threshold for per-video optical flow mean and filter out videos with no motion in them. In fact we analyze this scenario in the next section.


\captionexamples
\paragraph{Synthetic Captioning.} At a million-sample scale, it is not feasible to hand-annotate data points with prompts. Hence we resort to synthetic captioning to extract captions. However in light of recent insights on the importance of caption diversity~\citep{somepalli2023understanding} and taking potential failure cases of these synthetic captioning models into consideration, we extract \emph{three} captions per clip by using i) the image-only captioning model CoCa~\citep{pucetti2023training}, which describes spatial aspects well, ii) - to also capture temporal aspects - the video-captioner VideoBLIP~\citep{videoblip} and iii) to combine these two captions and like that, overcome potential flaws in each of them, a lightweight LLM. Examples of the resulting captions are shown in \Cref{fig:captionextable}. Concurrent works~\citep{wang2023internvid} have also explored summarizing framewise image captions with an LLM, which could also be a reasonable alternative.




% We find that although the captioner was train on image captions which are often static it can produce relevant video captions which can be used to train capable video-text models. We briefly show this in the next section however we le ave a deeper analysis into synthetic captioning methods for future work.

\paragraph{Caption similarities and Aesthetics.} Extracting CLIP~\citep{radford2021learning} image and text representations have proven to be very helpful for data curation in the image domain since computing the cosine similarity between the two allows for assessment of text-image alignment for a given example~\citep{schuhmann2022laion} and thus to filter out examples with erroneous captions. Moreover, it is possible to extract scores for visual aesthetics~\citep{schuhmann2022laion}. Although CLIP is only able to process images, and this consequently is only possible on a single frame level we opt to extract both CLIP-based i) text-image similarities and ii) aesthetics scores of the first, center, and last frames of each video clip. As shown in \Cref{subsec:data_curation,supsubsec:filtering_ablations}, using training text-video models on data curated by using these scores improves i) text following abilities and ii) visual quality of the generated samples compared to models trained on unfiltered data.


\paragraph{Text Detection.} 
In early experiments, we noticed that models trained on earlier versions of \datasetfiltered obtained a tendency to generate videos with excessive amounts of written text depicted which is arguably not a desired feat for a text-to-video model. To this end, we applied the off-the-shelf text-detector CRAFT~\citep{baek2019character} to annotate the start, middle, and end frames of each clip in our dataset with bounding box information on all written text. Using this information, we filtered out all clips with a total area of detected bounding boxes larger than 7\% to construct the final \datasetfiltered. 
\ocrvis
% We found that at a large scale, lots of samples contained unwanted text like subtitles or unwanted graphic overlays. In an attempt to filter this, we used CRAFT text-detection~\citep{baek2019character} to annotate the beginning, middle, and end frame of each video with bounding box information on all text that might be present. From this we computed an area ratio which determines what percentage of each annotated frame is covered by text-boxes, and filtered out the worst-offending samples as in other experiments.  

==> sec/appendices/D.tex <==
\section{Model and Implementation Details} \label{supsec:model_and_implementation_details}
\subsection{Diffusion Models} \label{subsec:diffusion_models}
%
In this section, we give a concise summary of DMs. We make use of the continuous-time DM framework~\citep{song2020score,karras2022elucidating}. 
Let $\pdata(\rvx_0)$ denote the data distribution and let $p(\rvx; \sigma)$ be the distribution obtained by adding i.i.d. $\sigma^2$-variance Gaussian noise to the data. Note that or sufficiently large $\sigma_{\mathrm{max}}$, $p(\rvx; \sigma_{\mathrm{max}^2}) \approx \gN\left(\bm{0}, \sigma_{\mathrm{max}^2}\right)$. DM uses this fact and, starting from high variance Gaussian noise $\rvx_M \sim\gN\left(\bm{0},\sigma_{\mathrm{max}^2}\right)$, sequentially denoise towards $\sigma_0=0$. In practice, this iterative refinement process can be implemented through the numerical simulation of the \emph{Probability Flow} ordinary differential equation (ODE)~\citep{song2020score}
%
\begin{align} \label{eq:probability_flow_ode}
    d\rvx = -\dot \sigma(t) \sigma(t) \nabla_\rvx \log p(\rvx; \sigma(t)) \, dt,
\end{align}
%
where $\nabla_\rvx \log p(\rvx; \sigma)$ is the \emph{score function}~\citep{hyvarinen2005estimation}. DM training reduces to learning a model $\vs_\vtheta(\rvx; \sigma)$ for the score function $\nabla_\rvx \log p(\rvx; \sigma)$. 
The model can, for example, be parameterized as $\nabla_\rvx \log p(\rvx; \sigma) \approx s_\vtheta(\rvx; \sigma) = (D_\vtheta(\rvx; \sigma) - \rvx)/ \sigma^2$~\citep{karras2022elucidating}, where $D_\vtheta$ is a learnable \emph{denoiser} that tries to predict the clean $\rvx_0$. 
The denoiser $D_\vtheta$ is trained via \emph{denoising score matching}~(DSM)
%
\begin{align} \label{eq:diffusion_objective}
    \E_{\substack{(\rvx_0, \rvc) \sim \pdata(\rvx_0, \rvc), (\sigma, \rvn) \sim p(\sigma, \rvn)}} \left[\lambda_\sigma \|D_\vtheta(\rvx_0 + \rvn; \sigma, \rvc) - \rvx_0 \|_2^2 \right],
\end{align}
%
where $p(\sigma, \rvn) = p(\sigma)\,\gN\left(\rvn; \bm{0}, \sigma^2\right)$, 
$p(\sigma)$ can be a probability distribution or density over noise levels $\sigma$. 
It is both possible to use a discrete set or a continuous range of noise levels. In this work, we use both options, which we further specify in \Cref{subsec:base_model_training_and_architecture}.   

$\lambda_\sigma \colon \R_+ \to \R_+$ is a weighting function, and $\rvc$ is an arbitrary conditioning signal. In this work, we follow the EDM-preconditioning framework~\citep{karras2022elucidating}, parameterizing the learnable denoiser $D_\vtheta$ as
%
\begin{align} \label{eq:edm_preconditioning}
    D_\vtheta(\rvx; \sigma) = \cskip(\sigma) \rvx + \cout(\sigma) F_\vtheta(\cin(\sigma) \rvx; \cnoise(\sigma)),
\end{align}
%
where $F_\vtheta$ is the network to be trained.

\textbf{Classifier-free guidance.} Classifier-free guidance~\citep{ho2022classifier} is a method used to guide the iterative refinement process of a DM towards a conditioning signal $\rvc$. The main idea is to mix the predictions of a conditional and an unconditional model
%
\begin{align} \label{eq:guidance}
    D^w(\rvx; \sigma, \rvc) = w D(\rvx; \sigma,\rvc) - (w - 1) D(\rvx; \sigma),
\end{align}
%
where $w \geq 0$ is the \emph{guidance strength}. The unconditional model can be trained jointly alongside the conditional model in a single network by randomly replacing the conditional signal $\rvc$ with a null embedding in~\Cref{eq:diffusion_objective}, e.g., 10\% of the time~\citep{ho2022classifier}. In this work, we use classifier-free guidance, for example, to guide video generation toward text conditioning.

% \subsection{Architecture Details} %\label{supsec:arch} NO SUBSECTION REF ALLOWED FOR NOW

% \hyperparams
% Due to the recent success and computational efficiency of latent diffusion models (LDM)~\cite{rombach2021high}, we choose our baseline model to come from that class. More specifically, we follow the architecture of~\cite{blattmann2023align}, which is an extension of LDM for the video domain and has shown strong results on text-to-video modeling. Thus we take a pretrained text2image model based on StableDiffusion2.1~\footnote{\url{https://github.com/Stability-AI/stablediffusion}} and add temporal attention and convolution layer in. Compared to~\cite{blattmann2023align} our baseline differs in three aspects: First, instead of only doing temporal finetuning~\cite{blattmann2023align},  we both train the spatial and temporal layers of the latent UNet~\cite{ronneberger2015u} based denoising autoencoder. Furthermore, to limit computational demands, we train all baselines on $256 \times 256$ px resolution instead of the original $320 \times 512$ px. Finally, since we have to crop the videos most of which have non-quadratic shapes, \cf \Cref{fig:resolutions_all}, we apply size- and crop-micro-conditioning~\cite{podell2023sdxl} to be able to generate center aligned videos at inference. Exact specifications of training and sampling hyperparameters can be found in \Cref{table:hyperparameters_ablation}.

\subsection{Base Model Training and Architecture} \label{subsec:base_model_training_and_architecture}
%
As discussed in~\label{sec:base-model}, we start the publicly available \emph{Stable Diffusion} 2.1~\citep{rombach2021high} (SD 2.1) model. In the EDM-framework~\citep{karras2022elucidating}, SD 2.1 has the following preconditioning functions:
%
\begin{align}
    \cskip^\mathrm{SD 2.1}(\sigma) &= 1, \\
    \cout^\mathrm{SD 2.1}(\sigma) &= -\sigma\,, \\
    % \cin^\mathrm{SD 2.1}(\sigma) &= \left( \sigma^2 + 1 \right)^{-0.5} \\
    \cin^\mathrm{SD 2.1}(\sigma) &= \frac{1}{\sqrt{\sigma^2 + 1}}\, ,  \\
    \cnoise^\mathrm{SD 2.1}(\sigma) &= \argmin_{j \in [1000]} (\sigma - \sigma_j)\,, \\
\end{align}
%
where $\sigma_{j+1} > \sigma_j$. The distribution over noise levels $p(\sigma)$ used for the original SD 2.1. training is a uniform distribution over the 1000 \emph{discrete} noise levels $\{\sigma_j\}_{j \in [1000]}$. One issue with the training of SD 2.1 (and in particular its noise distribution $p(\sigma)$) is that even for the maximum discrete noise level $\sigma_{1000}$ the \emph{signal-to-noise ratio}~\citep{kingma2021variational} is still relatively high which results in issues when, for example, generating very dark images~\citep{lin2023common,guttenberg2023diffusion}. \citet{guttenberg2023diffusion} proposed \emph{offset noise}, a modification of the training objective in~\Cref{eq:diffusion_objective} by making $p(\rvn \mid \sigma)$ non-isotropic Gaussian. In this work, we instead opt to modify the preconditioning functions and distribution over training noise levels altogether. 

\textbf{Image model finetuning.} We replace the above preconditioning functions with 
%
\begin{align}
    \cskip(\sigma) &= \left( \sigma^2 + 1 \right)^{-1}\,, \\
    \cout(\sigma) &=  \frac{-\sigma}{\sqrt{\sigma^2 + 1}}\,, \\
    \cin(\sigma) &= \frac{1}{\sqrt{\sigma^2 + 1}}\, , \\
    \cnoise(\sigma) &= 0.25 \log \sigma, \\
\end{align}
%
which can be recovered in the EDM framework~\citep{karras2022elucidating} by setting $\sigma_\mathrm{data} = 1$); the preconditioning functions were originally proposed in~\citep{salimans2022progressive}. We also use the noise distribution and weighting function proposed in~\citet{karras2022elucidating}, namely $\log \sigma \sim \gN(P_\mathrm{mean}, P_\mathrm{std}^2)$ and $\lambda(\sigma) = (1 + \sigma^2) \sigma^{-2}$, with $P_\mathrm{mean}=-1.2$ and $P_\mathrm{std}=1$. We then finetune the neural network backbone $F_\vtheta$ of SD2.1 for 31k iterations using this setup. For the first 1k iterations, we freeze all parameters of $F_\vtheta$ except for the time-embedding layer and train on SD2.1's original training resolution of $512 \times 512$. This allows the model to adapt to the new preconditioning functions without unnecessarily modifying the internal representations of $F_\vtheta$ too much. Afterward, we train all layers of $F_\vtheta$ for another 30k iterations on images of size $256 \times 384$, which is the resolution used in the initial stage of video pretraining. 

\textbf{Video pretraining.} We use the resulting model as the image backbone of our video model. We then insert temporal convolution and attention layers. In particular, we follow the exact setup from~\citep{blattmann2023align}, inserting a total of 656M new parameters into the UNet bumping its total size (spatial and temporal layers) to 1521M parameters. We then train the resulting UNet on 14 frames on resolution $256\times384$ for 150k iters using AdamW~\citep{loshchilov2017decoupled} with learning rate $10^{-4}$ and a batch size of 1536. We train the model for classifier-free guidance~\citep{ho2021classifierfree} and drop out the text-conditioning 15\% of the time. Afterward, we increase the spatial resolution to $320 \times 576$ and train for an additional 100k iterations, using the same settings as for the lower-resolution training except for a reduced batch size of 768 and a shift of the noise distribution towards more noise, in particular, we increase $P_\mathrm{mean} = 0$. During training, the base model and the high-resolution Text/Image-to-Video models are all conditioned on the input video's frame rate and motion score. This allows us to vary the amount of motion in a generated video at inference time.
%
\subsection{High-Resolution Text-to-Video Model} \label{subsec:high_resolution_text_to_video_model}
%
We finetune our base model on a high-quality dataset of $\sim$ 1M samples at resolution $576 \times 1024$. We train for $50k$ iterations at a batch size of 768, learning rate $3 \times 10^{-5}$, and set $P_\mathrm{mean} = 0.5$ and $P_\mathrm{std} = 1.4$. Additionally, we track an exponential moving average of the weights at a decay rate of 0.9999. The final checkpoint is chosen using a combination of visual inspection and human evaluation.
%
\subsection{High-Resolution Image-to-Video Model} \label{subsec:high_resolution_image_to_video_model}
%
We can finetune our base text-to-video model for the image-to-video task. In particular, during training, we use one additional frame on which the model is conditioned. We do not use text-conditioning but rather replace text embeddings fed into the base model with the CLIP image embedding of the conditioning frame. Additionally, we concatenate a noise-augmented~\citep{ho2021cascaded} version of the conditioning frame channel-wise to the input of the UNet~\cite{ronneberger2015u}. In particular, we add a small amount of noise of strength $\log \sigma \sim \gN(-3.0, 0.5^2)$ to the conditioning frame and then feed it through the standard SD 2.1 encoder. The mean of the encoder distribution is then concatenated to the input of the UNet (copied across the time axis). Initially, we finetune our base model for the image-to-video task on the base resolution ($320 \times 576$) for 50k iterations using a batch size of 768 and learning rate $3 \times 10^{-5}$. Since the conditioning signal is very strong, we again shift the noise distribution towards more noise, i.e., $P_\mathrm{mean} = 0.7$ and $P_\mathrm{std} = 1.6$. Afterwards, we fintune the base image-to-video model on a high-quality dataset of $\sim$ 1M samples at $576 \times 1024$ resolution. We train two versions: one to generate 14 frames and one to generate 25 frames. We train both models for $50k$ iterations at a batch size of 768, learning rate $3 \times 10^{-5}$, and set $P_\mathrm{mean} = 1.0$ and $P_\mathrm{std} = 1.6$. Additionally, we track an exponential moving average of the weights at a decay rate of 0.9999. The final checkpoints are chosen using a combination of visual inspection and human evaluation.
%
\subsubsection{Linearly Increasing Guidance} We occasionally found that standard vanilla classifier-free guidance~\citep{ho2021classifierfree} (see~\Cref{eq:guidance}) can lead to artifacts: too little guidance may result in inconsistency with the conditioning frame while too much guidance can result in oversaturation. Instead of using a constant guidance scale, we found it helpful to linearly increase the guidance scale across the frame axis (from small to high). A PyTorch implementation of this novel technique can be found in~\Cref{fig:linear_pred_guidance}.
\linearpredictioncode
\subsubsection{Camera Motion LoRA}
To facilitate controlled camera motion in image-to-video generation, we train a variety of \emph{camera motion LoRAs} within the temporal attention blocks of our model~\citep{guo2023animatediff}. In particular, we train low-rank matrices of rank 16 for 5k iterations. Additional samples can be found in~\Cref{fig:additional_motion_lora}.

% \subsection{Img2Vid Details} % \label{supsec:image_to_video_details} NO SUBSECTION REF ALLOWED FOR NOW

% \subsection{Img2Vid Distillation Details} % \label{supsec:image_to_video_distilation_details} NO SUBSECTION REF ALLOWED FOR NOW

\subsection{Interpolation Model Details} 
\label{supsubsec:interpolation_model_details} 
Similar to the text-to-video and image-to-video models, we finetune our interpolation model starting from the base text-to-video model, \cf \Cref{subsec:base_model_training_and_architecture}. To enable interpolation, we reduce the number of output frames from 14 to 5, of which we use the first and last as conditioning frames, which we feed to the UNet~\citep{ronneberger2015u} backbone of our model via the concat-conditioning-mechanism~\citep{rombach2021high}. To this end, we embed these frames into the latent space of our autoencoder, resulting in two image encodings $z_s,\, z_e \in \mathbb{R}^{c \times h \times w}$, where $c=4, \,h=52, \,w=128$. To form a latent frame sequence that is of the same shape as the noise input of the UNet, \ie $\mathbb{R}^{5 \times c \times h \times w}$, we use a learned mask embedding $z_m \in\mathbb{R}^{c \times h \times w}$ and form a latent sequence $ \boldsymbol{z} = \{z_s, z_m, z_m, z_m, z_e\}\in \mathbb{R}^{5 \times c \times h \times w}$. We concatenate this sequence channel-wise with the noise input and additionally with a binary mask where 1 indicates the presence of a conditioning frame and 0 that of a mask embedding. The final input for the UNet is thus of shape $\left( 5, 9, 52, 128 \right)$. In line with previous work~\citep{ho2022imagenvideo,singer2022make,blattmann2023align}, we use noise augmentation for the two conditioning frames, which we apply in the latent space. Moreover, we replace the CLIP text representation for the crossattention conditioning with the corresponding CLIP image representation of the start frame and end frame, which we concatenate to form a conditioning sequence of length 2.  

We train the model on our high-quality dataset at spatial resolution $576 \times 1024$ using AdamW~\citep{loshchilov2017decoupled} with a learning rate of $10^{-4}$ in combination with exponential moving averaging at decay rate 0.9999 and use a shifted noise schedule with  $P_\mathrm{mean}=1$ and $P_\mathrm{std}=1.2$. Surprisingly, we find this model, which we train with a comparably small batch size of 256, to converge extremely fast and to yield consistent and smooth outputs after only 10k iterations. We take this as another evidence of the usefulness of the learned motion representation our base text-to-video model has learned.   

\subsection{Multi-view generation}

We finetuned the high-resolution image-to-video model on our specific rendering of the Objaverse dataset. We render 21 frames per orbit of an object in the dataset at $576 \times 576$ resolution and finetune the 25-frame Image-to-Video model to generate these 21 frames. We feed one view of the object as the image condition. In addition, we feed the elevation of the camera as conditioning to the model. We first pass the elevation through a timestep embedding layer that embeds the sine and cosine of the elevation angle at various frequencies and concatenates them into a vector. This vector is finally concatenated to the overall vector condition of the UNet.


We trained for 12$k$ iterations with a total batch size of 16 across 8 A100 GPUs of 80GB VRAM at a learning rate of $1 \times 10^{-5}$.



==> sec/appendices/E.tex <==
\section{Experiment Details} \label{supsec:experiment_details}

\subsection{Details on Human Preference Assessment}
\label{supsubsec:human_eval}

For most of the evaluation conducted in this paper, we employ human evaluation as we observed it to contain the most reliable signal. For text-to-video tasks and all ablations conducted for the base model, we generate video samples from a list of 64 test prompts. We then employ human annotators to collect preference data on two axes: i) visual quality and ii) prompt following. More details on how the study was conducted~\Cref{supsubsubsec:human_eval_setup} and the rankings computed~\Cref{supsubsubsec:elo_score} are listed below.

\subsubsection{Experimental Setup}
\label{supsubsubsec:human_eval_setup}

Given all models in one ablation axis (\eg four models of varying aesthetic or motion scores), we compare each prompt for each pair of models (1v1). For every such comparison, we collect on average three votes per task from different annotators, i.e., \ three each for visual quality and prompt following, respectively. Performing a complete assessment between all pair-wise comparisons gives us robust and reliable signals on model performance trends and the effect of varying thresholds.
Sample interfaces that the annotators interact with are shown in~
\Cref{fig:humanevalserver}. The order of prompts and the order between models are fully randomized. Frequent attention checks are in place to ensure data quality.

\humanevalserver

\subsubsection{Elo Score Calculation}
\label{supsubsubsec:elo_score}
To calculate rankings when comparing more than two models based on 1v1 comparisons as outlined in \Cref{supsubsubsec:human_eval_setup}, we use Elo Scores (higher-is-better)~\citep{elo1978rating}, which were originally proposed as a scoring method for chess players but have more recently also been applied to compare instruction-tuned generative LLMs~\cite{bai2022training,askell2021general}. For a set of competing players with initial ratings $R_{\text{init}}$ participating in a series of zero-sum games, the Elo rating system updates the ratings of the two players involved in a particular game based on the expected and actual outcome of that game. Before the game with two players with ratings $R_1$ and $R_2$, the expected outcome for the two players is calculated as
\begin{align}
\label{eq:expected_elo}
E_1 =  \frac{1}{1 + 10^{\frac{R_2 - R_1}{400}}} \, , \\
E_2 =  \frac{1}{1 + 10^{\frac{R_1 - R_2}{400}}} \, . 
\end{align}
After observing the result of the game, the ratings $R_i$ are updated via the rule
\begin{align}
\label{eq:ranking_update}
R^{'}_{i} =  R_i + K \cdot \left(S_i - E_i \right), \quad i \in \{1,2\}
\end{align}
where $S_i$ indicates the outcome of the match for player $i$. In our case, we have $S_i=1$ if player $i$ wins and $S_i = 0$ if player $i$ loses. The constant $K$ can be seen as weight emphasizing more recent games. We choose $K=1$ and bootstrap the final Elo ranking for a given series of comparisons based on 1000 individual Elo ranking calculations in a randomly shuffled order. Before comparing the models, we choose the start rating for every model as $R_{\text{init}} = 1000$.     


\subsection{Details on Experiments from \Cref{sec:approach}} 
 
\subsubsection{Architectural Details}
Architecturally, all models trained for the presented analysis in \Cref{sec:approach} are identical. To insert create a temporal UNet~\citep{ronneberger2015u} based on an existing spatial model, we follow \citet{blattmann2023align} and add temporal convolution and (cross-)attention layers after each corresponding spatial layer. As a base 2D-UNet, we use the architecture from \emph{Stable Diffusion 2.1}, whose weights we further use to initialize the spatial layers for all runs except the second one presented in \Cref{fig:imageonly_comp}, where we intentionally skip this initialization to create a baseline for demonstrating the effect of image-pretraining. 
Unlike \citet{blattmann2023align}, we train all layers, including the spatial ones, and do not freeze the spatial layers after initialization. All models are trained with the AdamW~\citep{loshchilov2017decoupled} optimizer with a learning rate of $1.e-4$ and a batch size of $256$. Moreover, in contrast to our models from \Cref{sec:sota}, we do not translate the noise process to continuous time but use the standard linear schedule used in \emph{Stable Diffusion 2.1}, including offset noise~\citep{guttenberg2023diffusion}, in combination with the v-parameterization~\citep{ho2022classifier}. We omit the text-conditioning in 10\% of the cases to enable classifier-free guidance~\citep{ho2022classifier} during inference. 
To generate samples for the evaluations, we use 50 steps of the deterministic DDIM sampler~\citep{song2020improved} with a classifier guidance scale of 12 for all models. 

\subsubsection{Calibrating Filtering Thresholds}
\label{supsubsec:filtering_ablations}
\smallscaleablations
Here, we present the outcomes of our study on filtering thresholds presented in \Cref{subsec:data_curation}. As stated there, we conduct experiments for the optimal filtering threshold for each type of annotation while not filtering for any other types. The only difference here is our assessment of the most suitable captioning method, where we simply compare all used captioning methods. We train each model on videos consisting of 8 frames at resolution $256 \times 256$ for exactly 40k steps with a batch size of 256, roughly corresponding to 10M training examples seen during training. For evaluation, we create samples based on 64 pre-selected prompts for each model and conduct a human preference study as detailed in \Cref{supsubsec:human_eval}. \Cref{fig:filtering_ablations} shows the ranking results of these human preference studies for each annotation axis for spatiotemporal sample quality and prompt following. Additionally, we show an averaged `aggregated' score. 

For \emph{captioning}, we see that - surprisingly - the captions generated by the simple clip-based image captioning method CoCa of \citet{yu2022coca} clearly have the most beneficial influence on the model. However, since recent research recommends using more than one caption per training example, we sample one of the three distinct captions during training. We nonetheless reflect the outcome of this experiment by shifting the captioning sampling distribution towards CoCa captions by using $p_{\text{CoCa}} = 0.5; \, p_{\text{V-BLIP}} = 0.25; \,p_{\text{LLM}} = 0.25; \,$.

For \emph{motion filtering}, we choose to filter out 25\% of the most static examples. However, the aggregated preference score of the model trained with this filtering method does not rank as high in human preference as the non-filtered score. The rationale behind this is that non-filtered ranks best primarily because it ranks best in the category `prompt following' which is less important than the `quality' category when assessing the effect of motion filtering. Thus, we choose the 25\% threshold, as mentioned above, since it achieves both competitive performances in `prompt following' and `quality'. 

For \emph{aesthetics filtering}, where, as for motion thresholding, the `quality' category is more important than the `prompt following'-category, we choose to filter out the 25 \% with the lowest aesthetics score, while for \emph{CLIP-score thresholding} we omit even 50\% since the model trained with the corresponding threshold is performing best. Finally, we filter out the 25\% of samples with the largest text area covering the videos since it ranks highest both in the `quality' category and on average.

Using these filtering methods, we reduce the size of \dataset by more than a factor of 3, \cf \Cref{tab:subset_stats}, but obtain a much cleaner dataset as shown in \Cref{sec:approach}. For the remaining experiments in \Cref{subsec:data_curation}, we use the identical architecture and hyperparameters as stated above. We only vary the dataset as detailed in \Cref{subsec:data_curation}.


\subsubsection{Finetuning Experiments}
\label{supsubsec:finetune_exps}
For the finetuning experiments shown in \Cref{subsec:stage3}, we again follow the architecture, training hyperparameters, and sampling procedure stated at the beginning of this section. The only notable differences are the exchange of the dataset and the increase in resolution from the pretraining resolution $256 \times 256$ to $512 \times 512$ while still generating videos consisting of 8 frames. We train all models presented in this section for 50k steps.



\subsection{Human Eval vs SOTA}

For comparison of our image-to-video model with state-of-the-art models like Gen-2~\cite{gen2} and Pika~\cite{pika}, we randomly choose 64 conditioning images generated from a $1024 \times 576$ finetune of SDXL~\cite{podell2023sdxl}. We employ the same framework as in~\Cref{supsubsubsec:human_eval_setup} to evaluate and compare the visual quality generated samples with other models. 

For Gen-2, we sample the image-to-video model from the web UI. We fixed the same seed of 23, used the default motion value of 5 (on a scale of 10), and turned on the ``Interpolate" and ``Remove watermark" features. This results in 4-second samples at $1408 \times 768$. We then resize the shorter side to yield $1056 \times 576$ and perform a center-crop to match our resolution of $1024 \times 576$. For our model, we sample our 25-frame image-to-video finetune to give 28 frames and also interpolate using our interpolation model to yield samples of 3.89 seconds at 28 FPS. We crop the Gen-2 samples to 3.89 seconds to avoid biasing the annotators.


For Pika, we sample the image-to-video model from the Discord bot. We fixed the same seed of 23, used the motion value of 2 (on a scale of 0-4), and specified a 16:9 aspect ratio. This results in 3-second samples at $1024 \times 576$, which matches our resolution. For our model, we sample our 25-frame image-to-video finetune to give 28 frames and also interpolate using our interpolation model to yield samples of 3.89 seconds at 28 FPS. We crop our samples to 3 seconds to match Pika and avoid biasing the annotators. Since Pika samples have a small ``Pika Labs" watermark in the bottom right, we pad that region with black pixels for both Pika and our samples to also avoid bias.




% \todo{Needs details on exact questions etc, maybe take a look at VideoLDM paper, we even showed screenshots there} 


\subsection{UCF101 FVD} \label{supsec:ucf101_fvd}
%
This section describes the zero-shot UCF101 FVD computation of our base text-to-video model. The UCF101 dataset~\citep{soomro2012ucf101} consists of 13,320 video clips, which are classified into 101 action categories. All videos are of frame rate 25 FPS and resolution $240\times320$. To compute FVD, we generate 13,320 videos (16 frames at 25 FPS, classifier-free guidance with scale $w=7$) using the same distribution of action categories, that is, for example, 140 videos of ``TableTennisShot'', 105 videos of ``PlayingPiano'', etc. We condition the model directly on the action category (``TableTennisShot'', ``PlayingPiano'', etc.) and do not use any text modification. Our samples are generated at our model's native resolution $320 \times 576$ (16 frames), and we downsample to $240 \times 432$ using bilinear interpolation with antialiasing, followed by a center crop to $240 \times 320$. We extract features using a pretrained I3D action classification model~\citep{carreira2017quo}, in particular we are using a torchscript\footnote{\url{https://www.dropbox.com/s/ge9e5ujwgetktms/i3d_torchscript.pt} with keyword arguments \texttt{rescale=True, resize=True, return\_features=True}.} provided by~\citet{brooks2022generating}. 


\subsection{Additional Samples}
Here, we show additional samples for the models introduced in \Cref{sec:base-model,sec:txt2vid,sec:img2vid,sec:multiview}.

\subsubsection{Additional Text-to-Video Samples}
\additionaltexttwovideo
In \Cref{fig:additional_txt2vid}, we show additional samples from our text-to-video model introduced in~\Cref{sec:txt2vid}.
\subsubsection{Additional Image-to-Video Samples}
\additionalimagetwovideo
In \Cref{fig:additional_img2vid}, we show additional samples from our image-to-video model introduced in \Cref{sec:img2vid}.
\subsubsection{Additional Camera Motion LoRA Samples}
\additionalmotionlora
In \Cref{fig:additional_motion_lora}, we show additional samples for our motion LoRA's tuned for camera control as presented in \Cref{subsec:motion_lora}.
\subsubsection{Temporal Prompting via Temporal Cross-Attention Layers}
\additionaltemporalattention
Our architecture follows \citet{blattmann2023align}, who introduced dedicated temporal cross-attention layers, which are used interleaved with the spatial cross-attention layers of the standard 2D-UNet~\citep{dhariwal2021diffusion,ho2020ddpm}. During probing our Text-to-Video model from \Cref{sec:txt2vid}, we noticed that it is possible to independently prompt the model spatially and temporally by using different text-prompts as inputs for the spatial and temporal cross-attention conditionings, see \Cref{fig:additional_temporal_attention}. To achieve this, we use a dedicated spatial prompt to describe the general content of the scene to be depicted while the motion of that scene is fed to the model via a separate temporal prompt, which is the input to the temporal cross-attention layers. We provide an example of these first experiments indicating this implicit disentanglement of motion and content in \Cref{fig:additional_temporal_attention}, where we show that varying the temporal prompt while fixing random seed and spatial prompt leads to spatially similar scenes that obtain global motion properties following the temporal prompt.       

\subsubsection{Additional Samples on Multi-View Synthesis}
In \Cref{fig:additional_mv1,fig:additional_mv2,fig:additional_mv3,fig:additional_mv4}, we show additional visual examples for SVD-MV, trained on our renderings of Objaverse and MVImageNet datasets as described in \Cref{sec:multiview}.
\MVIone
\MVItwo
\MVIthree
\MVIfour


% \label{subsec:poseobjaverse}

% TIM Killed this section for now, make subsection in experiment details instead
% \section{Multi-view generation}
% \label{sec:MV}

